ALICE: An Automatic Design Flow for eFPGA Redaction

Fabricating an integrated circuit is becoming unaffordable for many semiconductor design houses. Outsourcing the fabrication to a third-party foundry requires methods to protect the intellectual property of the hardware designs. Designers can rely on embedded reconfigurable devices to completely hide the real functionality of selected design portions unless the configuration string (bitstream) is provided. However, selecting such portions and creating the corresponding reconfigurable fabrics are still open problems. We propose ALICE, a design flow that addresses the EDA challenges of this problem. ALICE partitions the RTL modules between one or more reconfigurable fabrics and the rest of the circuit, automating the generation of the corresponding redacted design.

==> clustering_pseudocode.tex <==
% I OMITTED CONTROL CHECKS 

\begin{algorithm}[t] \footnotesize
	\caption{Module Clustering}
	\label{alg:module-clustering}
	\DontPrintSemicolon % Some LaTeX compilers require you to use \dontprintsemicolon instead
	\KwIn{Max Input/Output size $maxIO$ and list of candidate modules $modules$}
	\KwOut{Set of all candidate clusters $clusters$}
	\Comment{Prerequisite: candidate modules must have an IO pin count $ \leq maxIO$}
	$clusters \gets []$\;
	\Comment{Initialize a cluster for each module}
	\For{ $m\gets0$ \KwInArray $modules$}{
        $clusters.append([m])$\;
    }
    
    $expanding \gets True$\;
    \While{$expanding$}{
        $expanging \gets False$\;
        $newClusters \gets []$ 
        \For{$c$ \KwInArray  }{
            $exp \gets FindExpansions(c, modules)$\;
            \For{$e$ \KwInArray exp}{
                $newClusters.append(c+e)$
            }
        }
    
    }
	
	\Return{$D$}	\;

\end{algorithm}

